TESLA Technical Design Report Part I: Executive Summary

The TESLA Technical Design Report Part I: Executive summary

==> tesla_cost.tex <==
\providecommand{\totalcost}{xxx}
\providecommand{\operating}{xxx}
\providecommand{\linaccost}{xxx}
\providecommand{\xfelacccost}{xxx}
\providecommand{\xfellabcost}{xxx}
\providecommand{\xfeltotalcost}{xxx}
\providecommand{\detcostone}{xxx}
\providecommand{\detcosttwo}{xxx}

\providecommand{\xfelcost}{xxx}

\providecommand{\personyears}{xxx}
\providecommand{\manpower}{xxx}

\providecommand{\gradientpercentage}{xxx}

\providecommand{\linea}{xxxx}
\providecommand{\lineb}{xxxx}
\providecommand{\linec}{xxxx}
\providecommand{\lined}{xxxx}
\providecommand{\linee}{xxxx}
\providecommand{\linef}{xxxx}
\providecommand{\lineg}{xxxx}
\providecommand{\lineh}{xxxx}

\providecommand{\linefela}{xxxx}
\providecommand{\linefelb}{xxxx}

\providecommand{\nfigure}[1]{}

